Robofleet: Open Source Communication and Management for Fleets of Autonomous Robots

Long-term deployment of a fleet of mobile robots requires reliable and secure two-way communication channels between individual robots and remote human operators for supervision and tasking. Existing open-source solutions to this problem degrade in performance in challenging real-world situations such as intermittent and low-bandwidth connectivity, do not provide security control options, and can be computationally expensive on hardware-constrained mobile robot platforms. In this paper, we present Robofleet, a lightweight open-source system which provides inter-robot communication, remote monitoring, and remote tasking for a fleet of ROS-enabled service-mobile robots that is designed with the practical goals of resilience to network variance and security control in mind. Robofleet supports multi-user, multi-robot communication via a central server. This architecture deduplicates network traffic between robots, significantly reducing overall network load when compared with native ROS communication. This server also functions as a single entrypoint into the system, enabling security control and user authentication. Individual robots run the lightweight Robofleet client, which is responsible for exchanging messages with the Robofleet server. It automatically adapts to adverse network conditions through backpressure monitoring as well as topic-level priority control, ensuring that safety-critical messages are successfully transmitted. Finally, the system includes a web-based visualization tool that can be run on any internet-connected, browser-enabled device to monitor and control the fleet. We compare Robofleet to existing methods of robotic communication, and demonstrate that it provides superior resilience to network variance while maintaining performance that exceeds that of widely-used systems.

==> introduction.tex <==
\section{INTRODUCTION AND RELATED WORK}

Remote management and tasking for service-mobile robots is essential to successful long-term deployments.
In practice, researchers are often responsible for building the systems and tooling necessary to accomplish these tasks themselves.
Robofleet aims to provide a simple, robust, and reusable solution to this problem, allowing researchers to focus on the deployments themselves rather than the infrastructure necessary to enable them.

When developing a system to enable long-term autonomous deployment, there are a number of explicit goals that need to be met.
First, the system needs to support persistent connection to multiple robots, as researchers will typically work with more than one robotic platform at a time.
The system must also support communication between robots, as well as two-way communication between the researchers and the robots, to enable successful monitoring and tasking. This communication needs to support a high density of traffic even in adverse conditions. The system must also be lightweight in terms of compute and network usage, as mobile robotic platforms are often constrained on both of these fronts. Finally, when communicating over the open internet, such a system needs to incorporate sufficient security and authorization controls.

Existing methods of enabling such deployment includes systems built on top of Rosbridge \cite{Crick2011RosbridgeRF}, a JSON-based transport layer allowing non-ROS clients to interact with ROS-based systems, and using native ROS with a remote ROS master. The core Rosbridge transport layer has critical performance and bandwidth consumption issues that limit these tools' practical use cases in network constrained environments. This internal issue was one of the key factors in the decision to develop Robofleet as a system independent from Rosbridge. A common alternative to Rosbridge is using the Robot Operating System (ROS) itself to facilitate communication. A shared ROS master can enable fast robot-to-robot communication when compared with Rosbridge. However, this architecture lacks authentication support, degrades in performance as the number of robots increases, and requires that all the machines in the system run ROS.

Robofleet provides several advantages over these existing systems. Robofleet adapts to adverse network conditions using backpressure monitoring. In addition, it supports configuration for rate limiting of topics combined with priority-based topic scheduling, ensuring that safety-critical messages take precedence over others. Such guarantees cannot be enforced in either Rosbridge or using native ROS. Its single-server architecture prevents duplication of message streams between robots, further decreasing network load in the case of multi-robot communication when compared with native ROS. Additionally, Robofleet uses a compact message format over WebSocket communication to minimize bandwidth usage and enable high throughput rates when compared with Rosbridge. Security control is another feature of Robofleet that is lacking in existing solutions. Specifically, Robofleet allows for topic-level access control, user authentication, and supports static IP address-based traffic control by leveraging a secure VPN. In addition to a central server, transport layer, and robot client, Robofleet includes a web-based visualizer and tasking tool tailored towards autonomous mobile robot deployment, which enables connection to the Robofleet system from any browser-enabled device. 

In this paper we describe the Robofleet system architecture, and compare it to existing state-of-the-art solutions for mobile robot communication. We provide experimental results to showcase Robofleet's superior performance in the case of adverse network conditions and multi-robot interactions. \SR{when experimental results are nailed down, provide some of the numeric results here}Agreed!. Robofleet is under active extension, and the source code can be found at \url{https://github.com/ut-amrl/robofleet}.


\section{related work}

There has been a significant amount of interest in this short-term communication task in the robotics community, resulting in a variety of widely-used tools to tackle some of these problems. Robot Web Tools includes an ecosystem of different tools that use the common Rosbridge transport layer \cite{toris2015robot}. These tools include visualization layers such as Ros2DJS, client libraries such as RosLibJS and RosLibPy, and interactive dashboards. There has also been recent research interest in developing interfaces for human operators to interact with fleets of remote robots \cite{Roldn2019MultirobotSV}. Each of these tools individually address some of the hurdles involved in successfully deploying autonomous robots, but stitching them together can itself involve overhead.

Beyond the explicit goals of monitoring and tasking, successfully sharing information between robots enables a wide variety of research initiatives beyond long-term autonomous deployment. Constructing a shared ``world model" between robots can allow them to succeed at a wide range of tasks \cite{waibel2011roboearth, mohanarajah2014rapyuta}. These works seek to allow robots to share information over long time scales, enabling them to tackle new tasks. By contrast, this paper will focus on the short-term, time-sensitive information exchange necessary to enable tasking and monitoring. In addition to long-term autonomous deployment, this style of communication is critical in many multi-agent systems, such as collaborative mapping tasks. For example, the Collaborative Visual SLAM algorithm would need some form of real-time communication between independent robotic agents in order to operate in real time \cite{CoSLAM}. An alternative approach to this task is to push computation to the cloud, as in \cite{CloudMapping}. Real-time inter-robot communication is also useful for teams of robots participating in tasks similar to those in RoboCup \cite{robocup97}, as well as for multi-agent online planning \cite{WU2011487}.
